Agent-Based Analysis of the Impact of Near Real-Time Data and Smart Balancing on the Frequency Stability of Power Systems

Single imbalance pricing provides an incentive to balance responsible parties (BRPs) to intentionally introduce power schedule deviations in order to reduce the control area imbalance and receive a remuneration through the imbalance settlement mechanism. This is called smart balancing or passive balancing and is actively encouraged in, e.g., the Netherlands and Belgium through the publication of near real-time (NRT) data on the control area imbalance by the transmission system operator. It is known that under certain conditions, smart balancing can deteriorate the frequency stability of the power system. This paper examines how the publication of different types of NRT data affects smart balancing and the frequency stability. A Monte-Carlo simulation of a dynamic multi-agent model is performed to analyse the effects of smart balancing with different parameters for the agents and the environment, using historical time series of the power imbalance of the German control block as a basis. It is found that smart balancing can significantly reduce the amount and cost of frequency restoration reserve activation, but leads to a general increase of the frequency variability. Depending on the type of NRT data and agent parameters, the frequency stability margins are also reduced. The negative effects on the frequency stability are stronger when NRT data is published using large bins and with long delays.

==> glossary.tex <==
\newacronym{tso}{TSO}{transmission system operator}
\newacronym{ca}{CA}{control area}
\newacronym[\glslongpluralkey={balance responsible parties}]{brp}{BRP}{balance responsible party}
\newacronym{ace}{ACE}{area control error}
\newacronym{isp}{ISP}{imbalance settlement period}
\newacronym[\glsshortpluralkey=FRR]{frr}{FRR}{frequency restoration reserve}
\newacronym{afrr}{aFRR}{automatic frequency restoration reserve}
\newacronym{mfrr}{mFRR}{manual frequency restoration reserve}
\newacronym{fcr}{FCR}{frequency containment reserve}
\newacronym{nrt}{NRT}{near real-time}
\newacronym{gcc}{GCC}{German grid control cooperation}
\newacronym{mas}{MAS}{multi-agent system}

==> highlights.tex <==
\item Novel dynamic agent-based model for smart balancing by balancing responsible parties
\item Analysis of effects of near real-time data and smart balancing on frequency stability
\item Identification of realistic smart balancing reactions and adverse stability effects
\item Agent and environmental parameter variations in a Monte-Carlo setting
\item Imbalance estimation and decision models based on multivariate Gaussian distributions

==> keywords.tex <==
smart balancing \sep power system stability \sep energy market design \sep frequency restoration reserve \sep imbalance settlement \sep  passive balancing 
